The Gittins Index: A Design Principle for Decision-Making Under Uncertainty

The Gittins index is a tool that optimally solves a variety of decision-making problems involving uncertainty, including multi-armed bandit problems, minimizing mean latency in queues, and search problems like the Pandora's box model. However, despite the above examples and later extensions thereof, the space of problems that the Gittins index can solve perfectly optimally is limited, and its definition is rather subtle compared to those of other multi-armed bandit algorithms. As a result, the Gittins index is often regarded as being primarily a concept of theoretical importance, rather than a practical tool for solving decision-making problems. The aim of this tutorial is to demonstrate that the Gittins index can be fruitfully applied to practical problems. We start by giving an example-driven introduction to the Gittins index, then walk through several examples of problems it solves - some optimally, some suboptimally but still with excellent performance. Two practical highlights in the latter category are applying the Gittins index to Bayesian optimization, and applying the Gittins index to minimizing tail latency in queues.

==> preamble.tex <==
\makeatletter

\usepackage{etoolbox}

\newtoggle{informs}
\@ifclassloaded{tut2016}{
  \toggletrue{informs}
}{
  \@ifclassloaded{tut2016_unofficial}{
    \toggletrue{informs}
  }{
    \togglefalse{informs}
  }
}
\newcommand{\ifinforms}{\iftoggle{informs}}

\newcommand{\RemoveLogos}{
  \def\@maketitleOneCol{%
    \newpage
    \vspace*{0.425in}%
    % no \theARTICLETOP
    \theCHAPTERNO
    \theARTICLETITLE
    \theSUBTITLE
    \theARTICLEAUTHORS
    \theARTICLEABSTRACT
    \theARTICLEKEYWORDS
    \theARTICLERULE
    \thispagestyle{headings}
  }
  \def\setoddRH{\hbox to \textwidth{\footnotesize\tabcolsep0pt
    \begin{tabular*}{\textwidth}[b]{l@{\extracolsep\fill}r}
    {\theRRHFirstLine} & \ThePage \\[-4pt]
    \rlap{\VRHDW{0.5pt}{0pt}{\textwidth}}&\\
    \end{tabular*}}}
  \def\setevenRH{\hbox to \textwidth{\footnotesize\tabcolsep0pt
    \begin{tabular*}{\textwidth}[b]{l@{\extracolsep\fill}r}
    \ThePage & {\theLRHFirstLine} \\[-4pt]
    \rlap{\VRHDW{0.5pt}{0pt}{\textwidth}}&\\
    \end{tabular*}}}
}

\PassOptionsToPackage{bb=ams}{mathalpha}

% requires packages bbold and bbold-type1 to avoid bitmap font
\ifinforms{
  \DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
  \DeclareSymbolFontAlphabet{\mathbbold}{bbold}
  \AtBeginDocument{\renewcommand{\1}{\mathbbold{1}}}
}{}

\ifinforms{
  \PassOptionsToPackage{labelfont=rm, font=small}{subcaption}
}{}

\usepackage[default, font=none, probability style=bb, ezeq number all, number within=section]{ezlib}
\usepackage{fontawesome}
\usepackage{xfp}
\usepackage{csquotes}
\usepackage{backref}
\usepackage{appendix}
\MakeOuterQuote{"}

% Nested nists all use the same bullet symbol
% Mostly for normal bulleted lists in `wide` paragraph-style lists
% (We don't have many/any actual nested lists)
% Using `\def` for compatibility with either INFORMS or non-INFORMS
\def\labelitemii{\labelitemi}
\def\labelitemiii{\labelitemi}
\def\labelitemiv{\labelitemi}

\newlength{\@bulletwidth}
\settowidth{\@bulletwidth}{\textbullet}

\def\labelitemi{\raisebox{0.125\@bulletwidth}{\scalebox{0.75}{\textbullet}}}

%\newcommand{\itemskipamount}{0.5\baselineskip}
\newcommand{\itemskipamount}{\baselineskip/3}
\setlist{topsep=\itemskipamount, itemsep=\itemskipamount}

\newcommand{\slscshape}{\fontfamily{lmr}\slshape\scshape\selectfont}
\DeclareTextFontCommand{\textslsc}{\slscshape}
\renewcommand{\eminnershape}{\slscshape}

% \newcommand{\textslsc}[1]{\begingroup\fontfamily{lmr}\slshape\scshape\selectfont#1\endgroup}

\renewcommand{\vec}{\v}

% From avt.sty
\renewmathcommand{\v}{\expandafter\boldsymbol} % vector
% \newcommand{\m}{\expandafter\mathbf} % matrix
% \declaremathcommand{\f}{\expandafter\operatorname} % function
% \renewmathcommand{\c}{\expandafter\mathcal} % calligraphic
% \newcommand{\bb}[1]{\in@{#1}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}\ifin@\mathbb{#1}\else\mathbbold{#1}\fi} % blackboard bold
\renewmathcommand{\t}{\expandafter\mathrel\expandafter\text} % text with spacing
% \newcommand{\h}[1]{\widehat{#1}} % hat
% \newcommand{\tl}[1]{\widetilde{#1}} % tilde

% In equations, `\text` should be upright, even if the surrounding text is e.g. italic
% Use `\textenv` to match the surrounding text
\let\textenv\text
\renewmathcommand{\text}{\textnormal}

\newcommandPIE{\smashop}[2][]{\ifstrempty{#1}{\smashoperator{#2#3#4#5}}{\smashoperator[#1]{#2#3#4#5}}}

\mathchardef\mhyphen="2D


% Section number and table of contents: go down to subsection
\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

% Don't force upshape numbers
\renewcommand{\@upn}{}

% Use full theorem/definition spacing around remarks
\def\th@remark{%
  \thm@headfont{\itshape}% heading
  \normalfont% body
}

\ifinforms{
  \cleartheorem{remark}
  \theoremstyle{definition}
  \newtheorem{remark}[theorem]{Remark}
}{}

\apptocmd{\@floatboxreset}{\centering}{}{error}
\apptocmd{\subcaption@iiminipage}{\centering}{}{error}

\pretocmd{\footnotemark}{\ifbool{hmode}{\unskip}{}}{}{error}
\pretocmd{\footnote}{\ifbool{hmode}{\unskip}{}}{}{error}

% Bibliography
\newcommand{\showURL}[1]{#1.}
\newcommand{\urlprefix}{}
\renewcommand{\bibsep}{\medskipamount}
\def\newblock{}%
\ifinforms{\newcommand{\BIBand}{and}}{}
\apptocmd{\thebibliography}{%
  \footnotesize%
  \def\newblock{}%
  \addcontentsline{toc}{section}{References}%
}{}{error}

\renewcommand*{\backrefalt}[4]{%
  \ifcase#1\or%
    Cited on page~#2.%
  \else%
    Cited on pages~#2.%
  \fi%
}

\AtBeginEnvironment{appendices}{%
  \crefalias{section}{appendix}%
  \crefalias{subsection}{appendix}%
  \crefalias{subsubsection}{appendix}%
}

\newlength{\default@topsep}
\setlength{\default@topsep}{\topsep}
\newenvironment{starquote}{\begin{itemize}[topsep=\default@topsep]\item[{(\ensuremath{\star})}]\em}{\end{itemize}}

\makeatother


\input{tikz-preamble}


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "gittins-tutorial"
%%% End:


==> tikz-preamble.tex <==
\makeatletter


\usepackage{tikz}
\usepackage{tikz-layers}
\usetikzlibrary{calc, decorations.pathreplacing}

\tikzset{
  every picture/.style={semithick, font=\small},
  axis/.style={semithick},
  axis tick/.style={semithick},
  guide/.style={thin, densely dashed, draw opacity=0.25},
  box line/.style={very thick, teal!75, line cap=round, rounded corners=0.125pt},
  box metal/.style={black!40},
  box fill/.style={teal!10},
  state/.style={circle, minimum width=2em, draw=teal!75, fill=teal!15, outer sep=0.3em},
  state selected/.style={circle, minimum width=2em, draw=teal!75, dashed, outer sep=0.3em},
  brace left/.style={
    decorate,
    decoration={
      brace,
      amplitude={\@braceamp},
      raise={\@braceraise},
    },
  },
  brace right/.style={
    decorate,
    decoration={
      brace,
      amplitude={\@braceamp},
      raise={\@braceraise},
      mirror,
    },
  },
}

\ifinforms{\tikzset{every picture/.style={scale=0.93}}}{}

\newcommand{\boxWidth}{1.3}
\newcommand{\boxHeight}{0.7}
\newcommand{\boxLidLength}{0.48}
\newcommand{\boxLidAngleClosedLeft}{0}
\newcommand{\boxLidAngleClosedRight}{0}
\newcommand{\boxLidAngleOpenLeft}{-107}
\newcommand{\boxLidAngleOpenRight}{107}

\newcommand{\drawBoxGeneric}[5][]{
  \draw[box line, #1]
  ($(#3) - 0.5*(#2)$)
  +($(0, 0 |- #2) ! \boxLidLength ! #4 : (#2)$)
  -- +(0, 0 |- #2)
  node[box metal] {\strut\textbullet}
  -- +(0, 0)
  -| +(#2)
  node[box metal] {\strut\textbullet}
  -- +($(#2) ! \boxLidLength ! #5 : (0, 0 |- #2)$);
}

\newcommand{\drawBoxFill}[3][]{
  \fill[box fill, #1] ($(#3) - 0.5*(#2)$) rectangle +(#2);
}

\newcommand{\drawBoxClosed}[2]{
  \drawBoxFill{\boxWidth, \boxHeight}{#1}
  \drawBoxGeneric{\boxWidth, \boxHeight}{#1}{\boxLidAngleClosedLeft}{\boxLidAngleClosedRight}
  \node[box metal] at ($(#1) + 0.5*(0, \boxHeight)$) {\strut\faLock};
  \drawBoxCaption{#1}{#2}
}

\newcommand{\drawBoxOpen}[2]{
  \drawBoxFill{\boxWidth, \boxHeight}{#1}
  \drawBoxGeneric{\boxWidth, \boxHeight}{#1}{\boxLidAngleOpenLeft}{\boxLidAngleOpenRight}
  \node[box metal] at ($(#1) + 0.5*(0, \boxHeight)$) {\strut\rlap{\faUnlock}\phantom{\faLock}};
  \drawBoxCaption{#1}{#2}
}

\newcommand{\drawBoxSelected}[2]{
  \drawBoxGeneric[dashed]{\boxWidth, \boxHeight}{#1}{\boxLidAngleOpenLeft}{\boxLidAngleOpenRight}
  \drawBoxCaption{#1}{#2}
}

\newcommand{\drawBoxCaption}[3][]{
  \ifstrempty{#3}{}{\node[align=center, #1] at (#2) {#3};}
}


% Guides

\newcommand{\tickSize}{1.25}

\NewDocumentCommand{\xguide}{ m m O{0, 0} }{
  \begin{scope}[on behind layer]
    \draw[axis tick] (#2 |- 0, 0) -- ++(0, {-\tickSize})
      \ifblank{#1}{}{++(#3) node[below] {#1}};
    \draw[guide] (#2 |- 0, 0) -- (#2);
  \end{scope}
}

\NewDocumentCommand{\yguide}{ s m m O{0, 0} }{
  \begin{scope}[on behind layer]
    \IfBooleanTF{#1}{
      \draw[axis tick] (#3 -| 0, 0) -- ++({\tickSize}, 0)
        \ifblank{#2}{}{++(#4) node[right] {#2}};
    }{
      \draw[axis tick] (#3 -| 0, 0) -- ++({-\tickSize}, 0)
        \ifblank{#2}{}{++(#4) node[left] {#2}};
    }
    \draw[guide] (#3 -| 0, 0) -- (#3);
  \end{scope}
}


% Local MDP value functions

\newcommand{\axisSize}{16.25}

\newcommand{\pictureLocalMdpValuePandora}[3]{%
  \begin{tikzpicture}[scale=0.18]
    \begin{scope}[on behind layer]
      \node[purple!50] at (#2, #2) {\faStar};
    \end{scope}

    % \draw[guide] (0, 0) -- +(\axisSize - 0.5, \axisSize - 0.5);

    \draw[axis, ->] (0, 0) -- (0, \axisSize) node[above] {$V_{\loc, #3}^*(\boxclosed; \alpha)$};
    \draw[axis, <->] (-\axisSize, 0) -- (\axisSize, 0) node[right] {$\alpha$};
    \draw[violet!85, very thick] (-\axisSize + 0.5, #1) -- (0, #1) -- (#2, #2) -- (\axisSize - 0.5, \axisSize - 0.5);

    \xguide{$0$}{0, 0}
    \xguide{$G_{#3}(\boxclosed) = #2$}{#2, #2}
    \ifstrequal{#1}{6}{
      \yguide*{$#1 = \E{v_{#3}} - c_{#3}$}{0, #1}[0, -0.5]
    }{
      \yguide*{$#1 = \E{v_{#3}} - c_{#3}$}{0, #1}[0, -0.25]
    }
    \yguide{$#2$}{#2, #2}
  \end{tikzpicture}%
}

\newcommand{\pictureLocalMdpValuePandoraOptional}[4]{%
  \ifnumcomp{\fpeval{trunc(#4, 0)}}{>}{6}{
    \tikzset{pandora take label/.style={below}}
  }{
    \tikzset{pandora take label/.style={above}}
  }
  \begin{tikzpicture}[scale=0.18]
    \renewcommand{\axisSize}{20}

    \begin{scope}[on behind layer]
      \node[purple!50] at (#2, #2) {\faStar};
    \end{scope}

    % \draw[guide] (0, 0) -- +(\axisSize - 0.5, \axisSize - 0.5);

    \draw[axis, ->] (0, 0) -- (0, \axisSize) node[above] {value};
    \draw[axis, <->] (-\axisSize * 0.23, 0) -- (\axisSize, 0) node[right] {$\alpha$};
    \draw[teal, very thick] (-\axisSize * 0.23 + 0.5, #1) -- (0, #1) -- (#2, #2) -- (\axisSize - 0.5, {#2 + (#2 - #1) / #2 * (\axisSize - 0.5 - #2)}) node[right] {\raisebox{-1.3em}{$V_{\loc, #3}^\opName(\boxclosed; \alpha)$}};
    \draw[orange!85!black, very thick] (-\axisSize * 0.23 + 0.5, #4) -- (\axisSize - 0.5, #4) node[pandora take label, fill=white, fill opacity=0.7, text opacity=1] {$V_{\loc, #3}^\tkName(\boxclosed; \alpha) = \E{v_{#3}} = #4$};
    \draw[lime!65!black, very thick] (-0.5, -0.5) -- (\axisSize - 0.5, \axisSize - 0.5) node[above=-0.2em] {$V_{\loc, #3}^\stName(\boxclosed; \alpha) = \alpha$};
    % \draw[violet!85, very thick] (-\axisSize + 0.5, #4) -- ({#2 - #2 / (#2 - #1) * (#2 - #4)}, #4) -- (#2, #2) -- (\axisSize - 0.5, \axisSize - 0.5) \node[right] {$V_{\loc, #3}(\boxclosed; \alpha)$};

    % \xguide{$0$}{0, 0}
    \xguide{$H_{#3} = \fpeval{#2 - #2 / (#2 - #1) * (#2 - #4)}$}{{#2 - #2 / (#2 - #1) * (#2 - #4)}, #4}
    \xguide{$G_{#3}(\boxclosed) = #2$}{#2, #2}
    % \yguide*{$#1 = \E{v_{#3}} - c_{#3}$}{0, #1}
    \yguide{$#2$}{#2, #2}
  \end{tikzpicture}%
}


% Braces

\newcommand{\@braceamp}{0.275em}
\newcommand{\@bracespace}{0.4em}
\newcommand{\@braceraise}{0.3em}
\newcommand{\@bracetrim}{0.3em}

% Usage: \braceleft[node style]{label}{xyLow}{xyHigh}
\newcommand{\braceleft}[4][]{
  \draw[brace left, #1] ($(#3) + (0, \@bracetrim)$) -- ($(#4) - (0, \@bracetrim)$);
  \node at ($(#3)!0.5!(#4)$) [align=right, left=\@bracespace] {#2};
}

% Usage: \braceright[node style]{label}{xyLow}{xyHigh}
\newcommand{\braceright}[4][]{
  \draw[brace right, #1] ($(#3) + (0, \@bracetrim)$) -- ($(#4) - (0, \@bracetrim)$);
  \node at ($(#3)!0.5!(#4)$) [align=left, right=\@bracespace] {#2};
}

% Usage: \braceabove[node style]{label}(xyLeft)(xyRight)
\newcommand{\braceabove}[4][]{
  \draw[brace left, #1] ($(#3) + (\@bracetrim, 0)$) -- ($(#4) - (\@bracetrim, 0)$);
  \node at ($(#3)!0.5!(#4)$) [align=center, above=\@bracespace] {#2};
}

% Usage: \bracebelow[node style]{label}(xyLeft)(xyRight)
\newcommand{\bracebelow}[4][]{
  \draw[brace right, #1] ($(#3) + (\@bracetrim, 0)$) -- ($(#4) - (\@bracetrim, 0)$);
  \node at ($(#3)!0.5!(#4)$) [align=center, below=\@bracespace] {#2};
}


\makeatother


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "gittins-tutorial"
%%% End:

